Space Efficient Breadth-First and Level Traversals of Consistent Global States of Parallel Programs

Enumerating consistent global states of a computation is a fundamental problem in parallel computing with applications to debug- ging, testing and runtime verification of parallel programs. Breadth-first search (BFS) enumeration is especially useful for these applications as it finds an erroneous consistent global state with the least number of events possible. The total number of executed events in a global state is called its rank. BFS also allows enumeration of all global states of a given rank or within a range of ranks. If a computation on n processes has m events per process on average, then the traditional BFS (Cooper-Marzullo and its variants) requires $\mathcal{O}(\frac{m^{n-1}}{n})$ space in the worst case, whereas ou r algorithm performs the BFS requires $\mathcal{O}(m^2n^2)$ space. Thus, we reduce the space complexity for BFS enumeration of consistent global states exponentially. and give the first polynomial space algorithm for this task. In our experimental evaluation of seven benchmarks, traditional BFS fails in many cases by exhausting the 2 GB heap space allowed to the JVM. In contrast, our implementation uses less than 60 MB memory and is also faster in many cases.

==> background.tex <==
\section{Background \& Terminology}
\label{sec:back}
%The basic concepts of posets and lattices are 
%now summarized .

We use the term {\em program} to represent a 
finite set of instructions, and {\em computation} to represent an execution of a program. In this paper, we 
restrict our focus to finite computations.  An event 
(of a computation) is a term that denotes --- 
depending on the context of the problem --- 
the execution 
of a single instruction or a collection of instructions
together.   
A parallel computation  
is a computation  involving more than one
processes/threads --- it is possible that the 
instructions executed by different processes/threads are
different. Hence, a distributed computation is a parallel 
 computation without shared memory
processes in which inter-process communication is possible 
only through message-passing. 
A computation is modeled as a set of events partially ordered by the Lamport's happened-before relation
\cite{Lamp:HappenBefore}. This partially ordered set (poset) of events is generally decomposed based on chains where each chain corresponds to execution on a single process/thread.
The happened-before
relation ($\ra$) on the set of events of a computation is the 
smallest relation that satisfies the following three 
conditions: $(1)$
If $a$ and $b$ are events in the same process 
and $a$ occurs before $b$, then $a \ra b$.  
$(2)$ For a distributed system, if $a$ is the sending
of a message and $b$ is the receipt of the same message, 
then $a \ra b$. For a shared memory system, if $a$ 
is the release of a lock by some thread and $b$ is the subsequent 
acquisition of that lock by any thread then $a \ra b$. $(3)$ If $a \ra b$ and $b \ra c$ then 
$a \ra c$. 


Formally, a finite partially ordered set ({\em poset} in short) 
 is
a pair $P = (E, \ra)$ where $E$ is a finite set and $\ra$ is 
an irreflexive, antisymmetric, and
transitive binary relation on $E$ \cite{davey}.
We obtain a poset when we apply the happened-before ($\ra$) on the set of events of a
finite computation. Let $E$ be the 
set of events. Consider two events $a, b \in E$. 
If either $a \ra b$ or $b \ra a$, we say that $a$ and $b$ are {\em comparable}; otherwise,
we say $a$ and $b$ are {\em incomparable} or {\em concurrent} (in the 
context of parallel computations), and denote this relation by $a~||~b$. Observe that $a~||~b~\wedge~b~||~c \not\Ra a~||~c$.   

It is important to note that 
multiple computations could have the identical posets as their model. 

\subsection{Concepts on Posets}

Let $P=(E,\ra)$ be a finite poset as defined above. 
A subset $Y\subseteq E$  is called an {\em chain (antichain)}, if every pair of distinct 
 points from $Y$ is comparable (incomparable) in $P$.
 The {\em height} of a poset
is defined to be the size of a largest chain in the poset.
 The {\em width} of a poset
is defined to be the size of a largest antichain in the poset.
All antichains of size equal to the width of the poset are called {\em width-antichains}
in this paper.
Let $\mathcal{A}(P)$ denote the set of all width-antichains
of $P$. Order $\leq$ is defined over $\mathcal{A}(P)$
as: \\
$A \leq B~~(A,B \in \mathcal{A}(P))$ iff $\forall a \in A, 
\exists b \in B: a \leq b$ in $P$. 

We model processes/threads 
as chains of posets, and thus 
events/states of every process/thread form a 
totally ordered chain.  %Under this context, 
A family $\pi=(C_i~|~i=1,2\ldots,n)$ of chains of $P$ 
is called a chain partition of $P$ if $\bigcup{C_i~
|~i=1,2\ldots,n)}=P$. 
%From here on, we would use chain partition in a stricter
%sense: to denote partitions $\pi$. 


Given a subset $Y \subseteq E$, the {\em meet} of $Y$, if it exists, is the greatest lower bound
of $Y$ and the {\em join} of $Y$ is the least upper bound.
%In Fig. \ref{fig:cuts}(i), the meet of the
%set $\{d,e\}$ is $a$. The meet of the set $\{b,c\}$ does not exist.
%An element is join-irreducible (meet-irreducible)
%if it cannot be expressed as join (meet) of other elements.
%In Fig. \ref{fig:cuts}(i), the elements $\{a,b,c\}$ are
%join-irreducible but $\{d,e,f\}$ are not.
A poset $P = (X, \leq)$ is a {\em lattice} if joins and meets exist for all
finite subsets of $X$.
%It is a {\em complete lattice} if joins and meets
%exists for all subsets of $X$. Since we deal only with finite posets in this paper, all lattices are trivially complete.
%The largest element of a lattice is called
%the {\em top} element.
Let $P$ be a poset with a given chain partition of width $w$.
In a parallel computation, $P$ is the set of events
executed under the happened-before partial order. Each chain would correspond to a
total order of events executed on a single process.
%The width of the poset is less than or equal to the number of processes.
In such a poset, every element $e$ can be identified with a tuple
$(i,k)$ which represents the $k$th event in the $i$th process; $1 \leq i \leq w$.

A subset $Q$ is a {\em downset} (also called {\em order ideal}), of $P$ if it satisfies the
constraint that if $f$ is in $Q$ and $e$ is less than or equal to $f$, then
$e$ is also in $Q$. 
%For any element $e \in P$, $D[e]$ is always a downset.
When a computation is modeled
as a poset of events, the downsets are called {\em consistent cuts}, or
{\em consistent global states} \cite{ChanLamp:Snap}. Throughout 
this paper, we use the term consistent cut. 
The set of downsets is closed under both union and intersection and
therefore forms a lattice under the set containment order \cite{davey}.
%Given two downsets $Q$ and $R$, their intersection (union)
%is simply the component-wise minimum (maximum) of the vectors for $Q$ and $R$.
%Similarly, the union is the component-wise maximum. 


==> evalold.tex <==
\newcommand{\our}{{\sf UniBFS}\xspace}
\newcommand{\bfs}{{\sf TBFS}\xspace}
\section{Experimental Evaluation}
\label{sec:eval}

\input{table/benchmarks}

We now present an experimental evaluation in which we compare the 
space and time taken by traditional BFS traversal of lattice 
of consistent cuts, against those taken by our implementation 
using the ideas presented in this paper. Note that the traditional BFS algorithm in \cite{CoopMarz:ConsDetGP} may enumerate the same global state multiple times.
In our evaluation, we optimize it as per \cite{cite:enumeratingglobal} to  enumerate every global state exactly once.

We conduct all the experiments on a Linux machine with an Intel Core i7 3.4GHz CPU, with L1, L2 and L3 
caches of size 32KB, 256KB, and 8192KB respectively. Both the implementations were compiled 
and ran running Oracle Java 1.7. 
The maximum heap size for Java virtual machine is limited to 2GB. We measure running time as wall-clock time measured in 
milliseconds (ms), and round it to seconds (s) for large values. We call our implementation of 
uniflow chain partition based BFS  \our, and denote the traditional BFS implementation by \bfs. 
For each 
 run of \our, 
we use Algorithm~\ref{alg:onlinepart} to find 
 the uniflow chain partition after sorting the events in the lexical order 
 of their vector clocks. 
When reporting runtimes for \our, we report the combined runtime of finding the uniflow chain partition 
of the poset, regeneration of vector clocks of events, and the lattice traversal.  

We use seven benchmark computations whose datails are shown in Table~\ref{tab:bench}. 
The column $n$ shows the original number of chains/processes in the computation, $|E|$
shows the number of events, $\cuts{E}$ shows the approximate number of consistent 
cuts in the lattice, and $n_u$ shows the number of chains in the uniflow chain partition 
that is computed by \our runs. The computations with the prefix {\em ``d-''} are randomly generated posets for modeling distributed computations. Each of them simulates a 
distributed computation on $n=10$ processes, with varying number of events: d-50 have 50 events, 
d-100 has 100, and d-300 has 300 events. After each internal event, every processes sends a message to a 
randomly selected process with a probability of 0.3. The benchmarks {\em bank}, and {\em hedc}  are computations obtained from real-world concurrent programs \cite{cite:bugpattern}, and are used by \cite{cite:jpredictor, cite:fasttrack, cite:datarace} for evaluating their predicate detection algorithms. The benchmark {\em bank} contains a typical error pattern in concurrent programs, and {\em hedc} is a web-crawler.
 Benchmarks starting with the prefix ``w-", w-4 and w-8, have 480 events distributed over  4 and 8 processes 
respectively. They 
help to highlight the influence of degree of parallelism on the performance of enumeration algorithms.


The runtime values of the two implementations are shown the last two columns of Table~\ref{tab:bench}. 
Note that for four benchmarks that generate large number of consistent cuts, \bfs (traditional BFS) 
runs out of the 2GB memory allocated to JVM. For the remaining three benchmarks, \our is slightly faster  
on smaller posets, and is within the same order of magnitude for a large poset. This is because large posets
generally lead to larger number of chains in uniflow partition, and our algorithm requires $\bigo{n_u^2}$ time 
per consistent cut, whereas \bfs takes $\bigo{n^2}$ time. 
Given that \bfs needs exponential space for the traversal, and cannot traverse posets with large lattices,  \our is extremely useful for such cases.  
The time taken in finding the uniflow chain partitions, and regenerating the 
vector clocks of the events is show in Figure~\ref{fig:vcgen}. As this result shows, 
we do not spend too much time in the pre-processing steps and most of the time is consumed 
by the traversal of the lattice. 

\begin{figure}
\centering
\includegraphics[scale=0.5]{figs/vcgen.pdf}
\caption{Time taken to compute uniflow partition and corresponding vector clocks.} 
\label{fig:vcgen}
\end{figure}

We also report the memory consumed by the both of implementations during the traversal.  Note that 
the memory consumed for \our involves the memory taken by vector clocks created for uniflow chain 
partition, as well as vectors created during the traversal. For both the implementations, the memory consumption reported is for the 
traversal of the lattice,  and does not include the 
memory required to store the original poset.  
For the three benchmarks for which \bfs does not run out of memory, the comparison of overall memory consumed 
during the traversal is shown in Figure~\ref{fig:mem}. Figure~\ref{fig:ourmem} shows the memory 
consumption for \our on the remaining benchmarks. 

\begin{figure}
\centering
\subfloat[Comparison: memory consumed by \bfs and \our]{
\includegraphics[scale=0.5]{figs/memory.pdf}
\label{fig:mem}
}
\qquad
\subfloat[Memory consumption for \our for remaining benchmarks 
on which \bfs fails]{
\includegraphics[scale=0.5]{figs/memour.pdf}
\label{fig:ourmem}
}
\caption{Memory consumption for traversing all the consistent cuts}
\end{figure}

\input{table/r25}
\input{table/r50}

We now show that our algorithm can be particularly effective in performing 
traversals of a given rank.   In Table~\ref{tab:r25}, and Table~\ref{tab:r50} we report the runtimes of the 
implementations when we only are interested in traversing the consistent 
cuts of rank 30 (30 events have been executed in the system), 
and rank 50. 
for the seven benchmarks. When traversing the lattice for consistent cuts of rank 30 result, on the five out of the seven benchmarks --- except w-4 and w-8 --- our 
\our significantly outperforms \bfs  for traversing the consistent cuts of this given rank. 
For rank 50, we outperform \bfs on all but one, except w-4, of the benchmarks.  


==> figs/nonuni_old.tex <==
\tikzstyle{place}=[circle,draw=black,fill=black,thick,inner sep=0pt,minimum size=2mm]
\tikzstyle{nsplace}=[circle,draw=black,thick,inner sep=0pt,minimum size=2mm]
\tikzstyle{place1}=[circle,draw=black,thick,inner sep=0pt,minimum size=3mm]
\tikzstyle{inner}=[circle,draw=black,fill=black,thick,inner sep=0pt,minimum size=1.25mm]
\tikzstyle{satlatnode}=[ellipse,draw=black,fill=black!20,thick,minimum size=5mm]
\tikzstyle{nsatlatnode}=[ellipse,style=dashed,thick]
\tikzstyle{satblock} = [rectangle, draw=gray, thin, fill=black!20,
text width=2.5em, text centered, rounded corners, minimum height=2em]
\tikzstyle{nsatblock} = [rectangle, draw=gray, thin,
text width=2.5em, text centered, rounded corners, minimum height=2em]
\tikzstyle{jbblock} = [rectangle, draw=black, thick, fill=black!20,
text width=2.5em, text centered, minimum height=2em]
\begin{figure}[!t]
\centering
%----
\subfloat[]{
\begin{tikzpicture}
\node at ( 0,1) [nsplace] [fill=blue!40] [label={above:{\small e}}]  (a) {};
\node at ( 1,1) [nsplace] [fill=blue!40] [label={above:{\small f}}] (b) {};
%\node at ( 0,1) [place] {};
\node at ( 0,0) [nsplace] [fill=orange!60] [label={below:{\small a}}] (e) {};
\node at ( 1,0) [nsplace] [fill=orange!60] [label={below:{\small b}}] (f) {};
\draw [thick,->] (a.east) -- (b.west);
\draw [thick,->] (e.east) -- (f.west);
\draw [thick,->] (a) -- (f);
\draw [thick,->] (e) -- (b);
\node at (-0.2, 1) [label=left:$P_{2}$] (bot1) {};
\node at (-0.2, 0) [label=left:$P_{1}$] (bot2) {};
\remove{
\node at (4,-.15) [label=below:$(b)$] (subref1) {};
%------- 4 procs ------
\node at ( 3.4,1) [nsplace] [fill=blue!40] (a2) {};
\node at ( 4.4,1) [nsplace] [fill=blue!40] (b2) {};
\node at ( 5.4,1) [nsplace] [fill=blue!40] (c2) {};
%\node at ( 0,1) [place] {};
\node at ( 3.4,0) [nsplace] [fill=orange!60] (e2) {};
\node at ( 4.4,0) [nsplace] [fill=orange!60] (f2) {};
\node at ( 5.4,0) [nsplace] [fill=orange!60] (g2) {};
\draw [thick,->] (a2.east) -- (b2.west);
\draw [thick,->] (b2.east) -- (c2.west);
\draw [thick,->] (e2.east) -- (f2.west);
\draw [thick,->] (f2.east) -- (g2.west);
\node at (3.3, 1) [label=left:$P_{1}$] (bot1) {};
\node at (3.3, 0) [label=left:$P_{2}$] (bot2) {};
\node at (3.4,-1) [nsplace] [fill=green!60] (a21) {};
\node at (4.4,-1) [nsplace] [fill=green!60] (b21) {};
\node at (5.4,-1) [nsplace] [fill=green!60] (c21) {};
%\node at ( 0,1) [place] {};
%\node at (3.4,-2) [nsplace] [] (e21) {};
%\node at (4.4,-2) [nsplace] [] (f21) {};
%\node at (5.4,-2) [nsplace] [] (g21) {};
\draw [thick,->] (a21.east) -- (b21.west);
\draw [thick,->] (b21.east) -- (c21.west);
%\draw [thick,->] (e21.east) -- (f21.west);
%\draw [thick,->] (f21.east) -- (g21.west);
\node at (3.3, -1) [label=left:$P_{3}$] (bot21) {};
%\node at (3.3, -2) [label=left:$P_{4}$] (bot22) {};
%\draw [thick,->] (f21) -- (b21);
\draw [thick,->] (a21) -- (f2);
%\draw [thick,->] (g21) -- (a2);
\draw [thick,->] (b2) -- (c21);
\node at (4,-1.15) [label=below:$(c)$] (subref3) {};
}
\end{tikzpicture}
}
\qquad
\subfloat[]{
\begin{tikzpicture}
\node at ( 0,0.5) [nsplace] [fill=blue!40] [label={\small e}] (a) {};
\node at ( 1,.5) [nsplace] [fill=blue!40] [label={right:{\small f}}](b) {};
%\node at ( 0,1) [place] {};
\node at ( 0,0) [nsplace] [fill=orange!60] [label={below:{\small a}}](e) {};
\node at ( 0.8,1) [nsplace] [fill=orange!60] [label={\small b}](f) {};
\draw [thick,->] (a.east) -- (b.west);
\draw [thick,->] (e.east) -- (f.south);
\draw [thick,->] (a) -- (f);
\draw [thick,->] (e.east) -- (b.south);
\node at (-0.1, 1) [label=left:$P_{3}$] (bot1) {};
\node at (-0.1, 0.5) [label=left:$P_{2}$] (bot2) {};
\node at (-0.1, 0) [label=left:$P_{1}$] (bot2) {};
\end{tikzpicture}
}
\qquad
\qquad
\subfloat[]{
\begin{tikzpicture}
\node at (0,1) [nsplace] [fill=blue!40] [label={above:{\small a}}] (a1) {};
\node at (0.8,1) [nsplace] [fill=blue!40] [label={above:{\small b}}](b1) {};
\node at (1.5,1) [nsplace] [fill=blue!40] [label={above:{\small c}}](c1) {};
%\node at ( 0,1) [place] {};
\node at (0,0) [nsplace] [fill=orange!60] [label={below:{\small e}}](e1) {};
\node at (0.6,0) [nsplace] [fill=orange!60] [label={below:{\small f}}] (f1) {};
\node at (1.5,0) [nsplace] [fill=orange!60] [label={below:{\small g}}](g1) {};
\draw [thick,->] (a1.east) -- (b1.west);
\draw [thick,->] (b1.east) -- (c1.west);
\draw [thick,->] (e1.east) -- (f1.west);
\draw [thick,->] (f1.east) -- (g1.west);
\node at (0, 1) [label=left:$P_{2}$] (bot11) {};
\node at (0, 0) [label=left:$P_{1}$] (bot12) {};
\draw [thick,->] (f1) -- (b1);
\draw [thick,->] (c1) -- (g1);
\end{tikzpicture}
}
\subfloat[]{
\begin{tikzpicture}
\node at (0,1) [nsplace] [fill=blue!40] [label={above:{\small a}}](a1) {};
\node at (0.8,1) [nsplace] [fill=blue!40] [label={above:{\small b}}](b1) {};
\node at (1.5,1) [nsplace] [fill=blue!40][label={above:{\small c}}] (c1) {};
%\node at ( 0,1) [place] {};
\node at (0,0) [nsplace] [fill=orange!60] [label={below:{\small e}}](e1) {};
\node at (0.6,0) [nsplace] [fill=orange!60] [label={below:{\small f}}] (f1) {};
\node at (2,1) [nsplace] [fill=orange!60] [label={above:{\small g}}](g1) {};
\draw [thick,->] (a1.east) -- (b1.west);
\draw [thick,->] (b1.east) -- (c1.west);
\draw [thick,->] (e1.east) -- (f1.west);
\draw [thick,->] (f1.east) -- (g1.south);
\node at (0, 1) [label=left:$P_{2}$] (bot11) {};
\node at (0, 0) [label=left:$P_{1}$] (bot12) {};
\draw [thick,->] (f1) -- (b1);
\draw [thick,->] (c1) -- (g1);
\end{tikzpicture}
}
\caption{Posets in (a) and (c) are not in uniflow partition: 
but (b) and (d) respectively are their equivalent uniflow partitions}
\label{fig:notuni}
\end{figure}


==> figs/onlinepart.tex <==
\tikzstyle{place}=[circle,draw=black,fill=black,thick,inner sep=0pt,minimum size=2mm]
\tikzstyle{nsplace}=[circle,draw=black,thick,inner sep=0pt,minimum size=2mm]
\tikzstyle{place1}=[circle,draw=black,thick,inner sep=0pt,minimum size=3mm]
\tikzstyle{inner}=[circle,draw=black,fill=black,thick,inner sep=0pt,minimum size=1.25mm]
\tikzstyle{satlatnode}=[ellipse,draw=black,fill=black!20,thick,minimum size=5mm]
\tikzstyle{nsatlatnode}=[ellipse,style=dashed,thick]
\tikzstyle{satblock} = [rectangle, draw=gray, thin, fill=black!20,
text width=2.5em, text centered, rounded corners, minimum height=2em]
\tikzstyle{nsatblock} = [rectangle, draw=gray, thin,
text width=2.5em, text centered, rounded corners, minimum height=2em]
\tikzstyle{jbblock} = [rectangle, draw=black, thick, fill=black!20,
text width=2.5em, text centered, minimum height=2em]
\begin{figure}[!t]
\centering
%----
\begin{tikzpicture}
\node at ( 0,1) [nsplace] [fill=blue!40] (a) {};
\node at ( 1.2,1) [nsplace] [fill=blue!40] (b) {};
%\node at ( 0,1) [place] {};
\node at ( 0,0) [nsplace] [fill=orange!60] (e) {};
\node at ( 1,0) [nsplace] [fill=orange!60] (f) {};
\draw [thick,->] (a.east) -- (b.west);
\draw [thick,->] (e.east) -- (f.west);
\draw [thick,->] (a) -- (f);
\draw [thick,->] (e) -- (b);
\node at (-0.2, 1) [label=left:$P_{2}$] (bot1) {};
\node at (-0.2, 0) [label=left:$P_{1}$] (bot2) {};
\node at (1, -0.15) [label=below:$(a)$] (subref) {};

\node at (3.5,0.5) [nsplace] [fill=blue!40] [label={above:{\footnotesize $[0,1,0]$}}] (a) {};
\node at ( 4.5,.5) [nsplace] [fill=blue!40] [label={above:$[0,2,1]$}] (b) {};
%\node at ( 0,1) [place] {};
\node at ( 3.5,0) [nsplace] [fill=orange!60] [label={above:$[0,0,1]$}] (e) {};
\node at ( 4.2,1) [nsplace] [fill=orange!60] [label={above:$[1,0,0]$}] (f) {};
\draw [thick,->] (a.east) -- (b.west);
\draw [thick,->] (e.east) -- (f.south);
\draw [thick,->] (a) -- (f);
\draw [thick,->] (e.east) -- (b.south);
\node at (3.4, 1) [label=left:$P_{3}$] (bot1) {};
\node at (3.4, 0.5) [label=left:$P_{2}$] (bot2) {};
\node at (3.4, 0) [label=left:$P_{1}$] (bot2) {};
\node at (4, -0.15) [label=below:$(b)$] (subref) {};
\end{tikzpicture}
\caption{Chain Partitions that are not Uniflow}
\label{fig:notuni}
\end{figure}


==> opts.tex <==
\section{Optimizations}
\label{sec:opt}

We discuss two optimizations: (a) the 
first optimization reduces the time taken per consistent cut by using
 additional space. (b) Then, we show    
that we can perform BFS traversal of the lattice without regenerating 
the vector clocks for uniflow chain partitions. This is particularly 
beneficial for 
 computations that execute large number of events, such that 
$|E| >> n$, and regeneration of vector clocks for uniflow chain  
partition may require large space.  
%This is achieved 
%at the expense of spending additional    
%time per consistent cut.  




==> table/rank50.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}lrrrr@{}}
\toprule
\multicolumn{1}{l}{Benchmark} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Rank 30\\ \bfs ~~~~     \our\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Rank 50\\ \bfs ~~~~    \our\end{tabular}} \\ \midrule
d-50                            & 1                                          & 2                                         & 3                                         & 4                                         \\
d-100                           & 5                                          & 6                                         & 7                                         & 8                                        
\end{tabular}
\label{tab:r50}
\caption{Comparison of rank traversal runtimes for $rank = 30$, and $rank = 50$.}
\end{table}


==> table/resultsbfs.tex <==
% Booktabs require to add \usepackage{booktabs} to your document preamble
\begin{table}[tbh]
\vspace{-.1in}
\center
\scriptsize
%\small
\tabcolsep=0.04in
\caption{The information of benchmarks and runtimes (sec.) of each algorithm.}
\label{table:benchmarkInfo}
\vspace{-.15in}
\begin{tabular}{@{}ccrr|rr|rr@{}}
\toprule
Benchmark         & $n$ & \multicolumn{1}{c}{$|E|$} & \multicolumn{1}{c}{\#cuts} & \multicolumn{1}{c}{BFS} & \multicolumn{1}{c}{Tree} & \multicolumn{1}{c}{Lex} & \multicolumn{1}{c}{QuickLex} \\\midrule
\textit{\textbf{d-300}}    & 10             & 300        & 4.2$\times10^7$        & 58.43                            & 3.80                              & 3.41                             & 0.76       \\
\textit{\textbf{d-500}}    & 10             & 500        & 2.3$\times10^8$    & 375.06                           & 19.40                             & 18.67                            & 3.78       \\
\textit{\textbf{bank}}     & 8              & 96         & 8$\times10^8$       & out of memory                    & 56.67                             & 64.37                            & 9.69       \\
\textit{\textbf{hedc}}     & 12             & 216        & 4.5$\times10^9$   & out of memory                    & 322.04                            & 488.22                           & 78.34      \\
\textit{\textbf{elevator}} & 12             & 38,528      & 2.7$\times10^{10}$  & out of memory                    & 2,248.39                          & 4,677.12                         & 660.40     \\
\textit{\textbf{w-4}}      & 4              & 480        & 9.4$\times10^6$         & 2.51                             & 0.88                              & 0.38                             & 0.16       \\
\textit{\textbf{w-8}}      & 8              & 480        & 7.4$\times10^9$     & out of memory                    & 609.74                            & 454.28                           & 128.03     \\\bottomrule
\end{tabular}
%\vspace{-.05in}
\end{table}






==> table/runtimes.tex <==
\begin{table}[]
\centering
\begin{tabular}{lrrrr}
\hline
Benchmark & $n$ & $|E|$ & $|\mathcal{C}(E)|$ & $n_u$ \\
\hline
d-50 & 10 & 50 & $\sim$ 0.6 million & 16 \\
d-100 & 10 & 100 & $\sim$ 1.2 million & 26 \\
w-4 & 4 & 480 & $\sim$ 9.3 million &  121\\
d-300 & 10 & 300 & $\sim$ 42.6 million & 68 \\
bank & 8 & 96 & $\sim$ 815 million &  8\\
hedc & 12 & 216 & $\sim$ 4.5 billion & 26  \\
w-8 & 8 & 480 & $\sim$7.3 billion & 63 
\end{tabular}
\caption{Description of benchmarks}
\label{tab:bench}
\end{table}

